D2.4 Report on the final prototype of programming abstractions for energy-efficient inter-process communication

Work package 2 (WP2) aims to develop libraries for energy-efficient inter-process communication and data sharing on the EXCESS platforms. The Deliverable D2.4 reports on the final prototype of programming abstractions for energy-efficient inter- process communication. Section 1 is the updated overview of the prototype of programming abstraction and devised power/energy models. The Section 2-6 contain the latest results of the four studies: i) GreenBST, a energy-efficient and concurrent search tree (cf. Section 2) ii) Customization methodology for implementation of streaming aggregation in embedded systems (cf. Section 3) iii) Energy Model on CPU for Lock-free Data-structures in Dynamic Environments (cf. Section 4.10) iv) A General and Validated Energy Complexity Model for Multithreaded Algorithms (cf. Section 5)

==> EPEM/conclusion.tex <==
In this study, we have devised a new general model for analyzing the energy complexity of multithreaded algorithms. The energy complexity of an algorithm is derived from its \textit{work}, \textit{span} and \textit{I/O} complexity.
Moreover, two case studies are conducted to demonstrate how to use the model to analyze the energy complexity of SpMV algorithms and matmul algorithms. The energy complexity analyses are validated for two SpMV algorithms and two matmul algorithm on two HPC platforms with different input matrices. The experimental results confirm the theoretical analysis with respect to which algorithm consumes more energy. The ICE energy complexity model gives algorithm-developers the insight into which algorithm is analytically more energy-efficient.
\comm{
In the future, we would extend our work in two directions:
\begin{itemize}
\item We want to develop a run-time framework which can choose the least energy-consuming implementations among the available kernels at run-time using the proposed energy model.
\item Nowadays, there are executable frameworks that connect different platforms to one task scheduler. Selecting the most energy-efficient platforms or system configurations to run applications is one of the techniques to achieve energy optimization. %Choosing the suitable platform to execute applications given an input can minimize energy consumption. 
In order to do so, the energy models need to be able to model the details of each platform. We want to improve the energy models to compare the energy consumption of applications between different platforms. 
\end{itemize}
}

==> intro-contribution.tex <==
The main achievements in this D2.4 report are summarized as follows.
\subsubsection{Libraries of Energy-efficient and Concurrent Data Structures}
%\remind{Contributions of Concurrent Data Structures}
In this section, we present a detailed description of GreenBST, an energy-efficient concurrent search tree that was 
briefly described in D2.3. Also in this deliverable,
GreenBST is tested with new state-of-the-art concurrent search trees that are not included in D2.3. The latest 
experimental results showed that GreenBST is more energy efficient and has 
higher throughput for both the concurrent search- and update- intensive workloads than the state-of-the-art. We also
have implemented GreenBST for Myriad2 platform and have conducted an experimental evaluation using the implementation.
\subsubsection{Customization methodology for implementation of streaming aggregation in embedded systems}
 In this section, we present a methodology for the customization of streaming aggregation implemented in modern low power embedded devices. The methodology is based on design space exploration and provides a set of customized implementations that can be used by developers to perform trade-offs between throughput, latency, memory and energy consumption. We compare the proposed embedded system implementations of the streaming aggregation operator with the corresponding HPC and GPGPU implementations in terms of performance per watt. Our results show that the implementations based on low power embedded systems provide up to 54 and 14 times higher performance per watt than the corresponding Intel Xeon and Radeon HD 6450 implementations, respectively. 
\subsubsection{Energy and Power Models}
\paragraph{Energy Model on CPU for Lock-free Data-structures in Dynamic Environments}
%\remind{Contribution summary of Energy Model on CPU for Lock-free Data-structures (Chalmers)}
Lock-free data structures are based on retry loops and are called by 
application-specific routines. In D2.3~\cite{EXCESS:D2.3}, we illustrate 
the performance impacting factors and the model that we use to cover a subset 
of the lock-free structures that we consider here. In the former study, the analysis 
is built upon properties that arise only when the sizes of the retry loops 
and the application-specific work are constant. 

In this section, we introduce two new frameworks that can be used to the 
capture the performance of a wider set of lock-free data structures (\textit{i.e.}\xspace the 
size of retry loops follow a probability distribution) in dynamic environments 
(\textit{i.e.}\xspace the size of application specific follows a probability distribution). 
These analyses allow us to estimate the energy consumption of an extensive set of 
lock-free data structures that are used under various access patterns.

\paragraph{Power Models Supporting Energy-Efficient Co-Design on Ultra-Low Power Embedded Systems}
This section is the complete report of RTHpower model on Myriad1 platform introduced previously in D2.3. In this version, the model is devised based on different training and test set of power data. The improved model provides more accurate power values for each components of Myriad1. 
\paragraph{A General and Validated Energy Complexity Model for Multithreaded Algorithms}
This study introduces a new general energy model ICE for analyzing the energy complexity of a wide range of multi-threaded algorithms. Compared to the EPEM model reported in D2.3, this model proposed using Ideal Cache memory model to compute I/O complexity of the algorithms. Besides a case study of SpMV to demonstrate how to apply the ICE model to find energy complexity of parallel algorithms, a case study for Dense Matrix Multiplication (matmul) is also conducted. The model is then validated with both data-intensive (i.e., SpMV) and computation-intensive (i.e., matmul) algorithms according to three aspects: different algorithms, different input types/sizes and different platforms.


==> uit-power-model.tex <==
\subsection{Introduction}
%The energy consumed by worldwide computing systems increases annually and becomes a major concern in information technology society. In order to tackle this issue, the research community and industry have proposed several research approaches to characterize the energy consumption of computing systems and applications \cite{Klavik14,Ciorba2014,Song2013,Gsch2014}.
%The energy consumed by worldwide computing systems increases annually and becomes a major concern in information technology society. 
%In order to tackle this issue, the scientific community and industry have proposed several research approaches to reduce the energy consumption of computing systems . 
%One of the key research directions to improve energy efficiency is to understand how much energy a computing system consumes and characterize the energy consumed by an individual component \cite{Orgerie2014}. 
%The energy and power consumption of computing systems can be either measured by integrated sensors or external multi-meters or estimated by models. Energy and power measurement equipment and sensors are not always available and can be costly to deploy and set up. Therefore, energy and power models are alternative and convenient methods to estimate the energy consumption of a computing component or a whole computing system \cite{Orgerie2014}.

Devising accurate power models is crucial to gain insights into how a computer system consumes power and energy. By knowing the energy consumption of individual components on a specific computing architecture, researchers and practitioners can design and implement new approaches to reduce the energy consumed by a certain algorithm on a specific platform \cite{Umar2016, Umar:2015,Umar20162,Lagraviere2016}.
Significant efforts have been devoted to devising power and energy models, resulting in several seminal papers in the literature, such as \cite{jacobson2011, Leng:2013, MCPAT, Alonso2014, Choi2013, Choi2014, Korthikanti2009, Korthikanti2010, 7108419, Mishra:2015, Snowdon:2009} modeling power of architectures or applications. 

Jacobson et al. \cite{jacobson2011} proposed accurate power modeling methodologies for POWER-family processors while GPUWattch \cite{Leng:2013} and McPAT \cite{MCPAT} are robust power models for GPUs and CPUs. Alonso et al. \cite{Alonso2014} proposed energy models for three key dense-matrix factorizations. 
% Kor, Choi devise general energy models which can estimate energy consumption of several applications. Roofline model by Choi ... 
Roofline model of energy \cite{Choi2013, Choi2014} considers both algorithmic and platform properties. However, the Roofline model does not consider the number of cores running applications as a model parameter (i.e., coarse-grained models). Theoretical models by Korthikanti et al. \cite{Korthikanti2009, Korthikanti2010} are based on strong theoretical assumptions and are not yet validated on real platforms. Koala model \cite{Snowdon:2009} requires the system supported dynamic voltage and frequency scaling (DVFS) and short frequency switching delay in order to gain energy saving from its methodology. Only two x86-based platforms among 10 validated platforms gain energy saving results which are presented in the paper. Imes et al. \cite{7108419} provided a portable approach to make real-time decision and run the chosen configuration to minimize energy consumption. However, the approach requires systems supporting hardware resource (e.g., model-specific register) to expose energy data to the software during run-time. Mishra et al. \cite{Mishra:2015} used probabilistic approach to find the most energy-efficient configuration by combining online and offline machine-learning approaches. This approach requires a significant data collected to feed to its probabilistic network. %The modeling approach proposed in this study is lightweight and applicable to any ultra-low power embedded systems as long as there is a mean to measure the energy consumption of micro-benchmarks on the targeted platform. 
%The details of existing energy and power models are described in Section \ref{sec:RelatedWorks}. 

Recently, ultra-low power (ULP) embedded systems have become popular in the scientific community and industry, especially in media and wearable computing. ULP embedded systems have different architecture from the general-purpose architectures (e.g., CPU and GPU). As the result, the approach to model the power of ULP systems needs to be customized for their architecture. ULP systems can achieve low energy per instruction down to a few pJ \cite{Alioto2012}. Alioto \cite{Alioto2012} mentioned that techniques such as pipe-lining, hardware replication, ultra-low-voltage memory design and leakage-reducing make a system ultra-low power. In order to model ULP systems where energy per instruction can be as low as few pJ, more accurate fine-grained approaches are needed. For instance, the dynamic power $P^{dyn}$ of operations in Table \ref{table:Punits}, which is as low as 13 mW, cannot be measured by using the prior coarse-grained approaches. 

Two of the most popular strategies to reduce the energy consumption are Dynamic Voltage/Frequency Scaling (DVFS) \cite{LeSueur2010} and race-to-halt (RTH) (i.e, system is run as fast as possible, and then switched to idle state to save energy) \cite{Awan2014}. For new embedded systems which do not support DVFS features such as Movidius Myriad1 \cite{7006377}, RTH is one of remaining choices for saving energy. In fact, Myriad1 supports a power management feature to power on/off individual cores. RTH strategy says that the system should execute the application as fast as possible and then go to sleep to save energy. For ultra-low power embedded systems, RTH might not be always true.  
However, to the best of our knowledge, there are no power models that supports investigating the trade-off between performance and energy consumption on ULP embedded system, 
%and provide insight into how an application consumes energy 
and, particularly, whether the RTH strategy that is widely used in high-performance computing (HPC) systems is still applicable to ULP embedded systems.  
 
In this study, we propose new RTHpower models which support architecture-application co-design by considering both platform and application properties. %The models provide insights into how an application consumes energy when running on an ULP embedded system, particularly Movidius Myriad1 \cite{7006377}. 
The RTHpower models are application-general since they characterize applications by their operational intensity \cite{Williams2009} which can be extracted from any application. The RTHpower models are also practical since they are built and validated on Movidius platform with application kernels.
%The RTHpower models are able to predict when to use RTH for a given application on an ultra-low power embedded system. We also present an application scenario where RTH no longer works.  The new RTHpower models can indicate whether the RTH strategy is an energy-efficient approach for a given application running on the ULP embedded system.

The contributions of this study are three-fold as follows:
\begin{itemize}
\item We propose new application-general fine-grained power models (namely, RTHpower) that provide insights into how a given application consumes power and give hints to investigate the trade-offs between performance and power consumption on ULP embedded systems. The RTHpower models support co-design on ULP systems by considering three parameter groups: platform properties, application properties (e.g., operational intensity and scalability) and execution settings (e.g., the number of cores executing a given application) (cf. Section \ref{sec:PowerModel}). %The models are able to estimate the power consumed by an application running with a specific number of cores and can be used to calculate how many cores to run the application to consume the least energy. 
%By considering both platform and application properties, the models give more insights into how to design applications to achieve better energy efficiency (cf. Section \ref{sec:PowerModel}).
\item We validate the new RTHpower models on an ultra-low power embedded system, namely Movidius Myriad1. The models are trained and validated with power data from different sets of micro-benchmarks, two popular kernels from Berkeley dwarfs \cite{Asa06} and one data-intensive kernel from Graph500 benchmarks \cite{6114175}. The three chosen application kernels are dense matrix multiplication (Matmul), sparse matrix vector multiplication (SpMV) and breadth first search (BFS). The model validation has percentage error at most 8.5\% for micro-benchmarks and 12\% for application kernels (cf. Section \ref{sec:Validation}). 
%%%%%%%Note that although the RTHpower models are validated on a specific system (i.e., Myriad1), the procedure to retrieve the models parameters is applicable to other ULP embedded systems as long as there is a mean to measure the energy consumption of micro-benchmarks on the systems.
\item We investigate the RTH strategy on an ultra-low power embedded platform using the new RTHpower models. We propose a framework that is able to predict whether the RTH strategy minimizes energy consumption for a given application. We validate the framework using micro-benchmarks and application  kernels and show that the framework prediction is accurate. From our experiments, we show real scenarios when to use RTH and when not to use RTH. We can save up to 61\% energy for dense matrix multiplication, 59\% energy for SpMV by using RTH and up to 5\% energy for BFS by not using RTH (cf. Section \ref{sec:Framework}).
\end{itemize}
\subsection{Movidius Myriad1 Platform}
\label{sec:Architecture}
This section describes briefly Myriad1 platform which is used to devise and validate the new RTHpower models. Myriad1 is developed by Movidius company and belongs to a new generation of ultra-low power processors in mobile computing industry \cite{7006377}. Myriad1 does not support DVFS. 

In terms of processors, Myriad1 chip contains eight separate SHAVE (Streaming Hybrid Architecture Vector Engine) cores and one RISC core named LEON. Each SHAVE core resides on one solitary power island.
A SHAVE core contains a set of register files (e.g., IRF, SRF and VRF) and a set of operation units, including arithmetic units (e.g., IAU for integer, SAU for scalar, VAU for vector) and load/store units (e.g., LSU0 and LSU1). The architecture of a SHAVE core is shown in Figure \ref{fig:ShaveInstructionUnits}. Eight SHAVE cores can access Double Data Rate Random Access Memory (DDR RAM) via L2 cache or bypass L2 cache.
\begin{figure}[!t] \centering
\resizebox{0.75\columnwidth}{!}{ \includegraphics{figures/ShaveInstructionUnits-2.png}}
\caption{SHAVE Operation Units}
\label{fig:ShaveInstructionUnits}
\end{figure}

In this work, we consider the register files and operation units as described in Table \ref{table:ShaveComponents}.
\begin{table}
\caption{Descriptions of SHAVE Components}
\label{table:ShaveComponents}
\begin{center}
\begin{tabular}{ll}
\hline\noalign{\smallskip}
Component & Description\\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
IRF & Integer register file\\
SRF & Scalar register file\\
VRF & Vector register file\\
IAU & Perform integer arithmetic operations\\
SAU & Perform scalar integer/floating point arithmetic operations\\
VAU & Perform vector integer/floating point arithmetic operations\\
LSU0 & Perform memory access and IO instructions\\
LSU1 & Perform memory access and IO instructions\\
CMU & Compare/Move data among register files\\
PEU & Predicated execution unit\\
BRU & Branch/Repeat Unit\\
\noalign{\smallskip}\hline
\end{tabular}
\end{center}
\end{table}
Myriad1 platform has an ultra-low power design \cite{Myriad:2015}. Myriad1 can provide theoretical peak energy efficiency at 45 Gflops/Watt \cite{7006377}. It supports power management allowing individual cores to be powered on/off. However, the trade-off of Myriad1 energy efficiency is its difficulty to program. In order to achieve high energy efficiency, programmers have to write programs in an assembly language \cite{7006377} and control instruction pipelines and direct memory access (DMA) transfers between different memory modules. The scheduling part and computation part of applications are written on separate code files. The scheduling part is on LEON core and the computation part is on SHAVE cores.
The compiler is a subset of GCC compiler and therefore, not all libraries are supported. This high complexity to program is also noticed in other ULP systems \cite{Phothilimthana:2014}.
\subsubsection{Measurement Set-up}
We use a bench setup consisting of one Myriad1 MV153 board, one DC step down converter and one HAMEG multimeter to measure voltage, current and consumed power. The MV153 board is modified as shown in Figure \ref{fig:PowerSupplyModification} in order to measure the voltage, current and consumed power of only Myriad1 chip instead of the whole board. The two power output sources from the chip are connected to the HAMEG multimeter. %%%%%%The HAMEG multimeter provides the measured data at a rate of approximately 50 times per second and be able to capture the measurements for benchmarks with the execution time longer than 20 milliseconds.
\subsubsection{Micro-benchmarking Methodology}
%A \emph{micro-benchmark} in this work is a small piece of assembly code designed to measure the performance or power of a hardware unit or an operation. For each micro-benchmark, a number of operations is infinitely repeated so that their consumed power can be measured. This convention enables the comparisons among SHAVE units. The number of instructions in one iteration for each mico-benchmark is calculated so that the whole iteration fits to L1 cache (1KB).
We design different micro-benchmark suites and run each micro-benchmark with different numbers of cores (i.e., 1, 2, 4 and 8) to collect the power data. The micro-benchmarks are written in assembly language (ASM) to make the experimental results close to the actual hardware performance. In this study, we create a set of 35 micro-benchmarks categorized in two groups, i.e., arithmetic micro-benchmarks and intensity-based micro-benchmarks. 
Each arithmetic micro-benchmark runs one or multiple arithmetic units in parallel. For instance, SauXor runs exclusive-OR instruction on SAU unit. The intensity-based micro-benchmarks run both arithmetic unit and load store unit to simulate real applications. The ratio of arithmetic instructions to load-store instructions identifies the operational intensity of micro-benchmarks. %We measure the power consumption of Myriad1 chip when running each micro-benchmark with different numbers of cores (i.e., 1, 2, 4 and 8) to collect the power data. 
The micro-benchmark suites are elaborated more in Section \ref{sec:model-validation-micro}.
%The model is trained using the measured results from designed micro-benchmarks. 'Bottom-up ones divide the architecture into power components and predict their stand- alone power consumption to later derive the overall power consumption. The Bottom-up approaches rely on some knowledge of the underlying architecture to produce more reliable and enlightening power models. For instance, they can provide a microarchitectural component-wise power consumption breakdown.'
%The platform supports the measurement of the power consumed by the chip only. The modifications were made to the MV153 board to bypass the on-board voltage regulator which down-regulates the 5V wall PSU to the 1.2V core voltage required by Myriad1 chip as Figure \ref{fig:PowerSupplyModification}. 
\begin{figure}[!t] \centering
\resizebox{0.8\columnwidth}{!}{ \includegraphics{figures/PowerSupplyModification.png}}
\caption{Myriad1 Power Supply Modification}
\label{fig:PowerSupplyModification}
\end{figure}
\subsection{RTHpower - Analytical Power Models}
\label{sec:PowerModel}
We first present a new power model for operation units and then develop it to the RTHpower models considering application properties.
\subsubsection{A Power Model for Operation Units}
The experimental results of the micro-benchmarks suite for operation units show that the power consumption of Movidius Myriad1 platform is ruled by Equation \ref{eq:Pfirst}. In the equation, the static power $P^{sta}$ is the required power when the Myriad1 chip is on, including memory storage power; the active power $P^{act}$ is the power consumed when a core is on and actively performing computation work; the dynamic power $P^{dyn}(op)$ is the power consumed by each operation unit such as arithmetic units (e.g., IAU, VAU, SAU, CMU) or load/store units (e.g., LSU0, LSU1) in one SHAVE.  The experimental results show that different operations have different $P^{dyn}(op)$ values as listed in Table \ref{table:Punits}. Total dynamic power of a core is the sum of all dynamic power from involved units. If benchmarks or programs are executed with $n$ cores, the active and dynamic power needs to be multiplied with the number of used cores. By using regression fitting techniques, the average value of $P^{sta}$ and $P^{act}$ from all micro-benchmarks are computed in Equation \ref{eq:Pstat1} and Equation \ref{eq:Pstat2}. For ULP system such as Myriad1, $P^{sta}$ is significant low with only 62.125 mW. Table \ref{table:Parameters} provides the description of parameters in the proposed models. 
\begin{equation} \label{eq:Pfirst}
	P^{units}=P^{sta}+ n \times \left(P^{act} + \sum_i{P^{dyn}_i(op)} \right)
\end{equation}
\begin{equation} \label{eq:Pstat1}
	P^{sta}=62.125 \text{ mW}
\end{equation}
\begin{equation} \label{eq:Pstat2}
	P^{act}=30 \text{ mW}
\end{equation}
\begin{table}
\caption{\textbf{$P^{dyn}(op)$} of SHAVE Operations}
\label{table:Punits}
\begin{center}
\begin{tabular}{lll}
\hline\noalign{\smallskip}
Operation & Description & $P^{dyn}$ (mW)\\ 
\noalign{\smallskip}\hline\noalign{\smallskip}
SAUXOR  &  Perform bitwise exclusive-OR on scalar              & 15          \\ 
SAUMUL  &  Perform scalar multiplication               & 18          \\ 
VAUXOR  &  Perform bitwise exclusive-OR on vector               & 35.6         \\
VAUMUL  &  Perform vector multiplication             & 52.6 \\ 
IAUXOR  &  Perform bitwise exclusive-OR on integer              & 15          \\ 
IAUMUL  &  Perform integer multiplication              & 21          \\ 
CMUCPSS &  Copy scalar to scalar             & 20          \\ 
CMUCPIVR&  Copy integer to vector              & 13         \\ 
LSULOAD &  Load from a memory address to a register            & 28         \\ 
LSUSTORE&  Store from a register to a memory address              & 37         \\
\noalign{\smallskip}\hline
\end{tabular}
\end{center}
\end{table}
\begin{table}
\caption{Model Parameter List}
\label{table:Parameters}
\begin{center}
\begin{tabular}{ll}
\hline\noalign{\smallskip}
Parameter & Description \\
\noalign{\smallskip}\hline\noalign{\smallskip}
$P^{sta}$                & Static power of a whole chip         \\ 
$P^{act}$                 & Active power of a core        \\ 
$P^{dyn}(op)$                  & Dynamic power of an operation unit        \\ 
$P^{LSU}$                  & Dynamic power of Load Store Unit          \\ 
$P^{ctn}$                  & Contention power of a core waiting for data          \\ 
$m$                 & Average number of active cores accessing data       \\ 
$n$                & Number of assigned cores to the program      \\ 
$I$              & Operational intensity of an application         \\ 
$\alpha$                & Time ratio of data transfer to computation       \\
%$\beta$ & Online-learning parameter of an application\\
\noalign{\smallskip}\hline\noalign{\smallskip}
\end{tabular}
\end{center}
\end{table}
\subsubsection{RTHpower Models for Applications}
\label{sec:ModelEquation}
Since typical applications require both computation and data movement, we use the concept of operational intensity proposed by Williams et al. \cite{Williams2009} to characterize applications. An application can be characterized by the amount of computational work $W$ and data transfer $Q$. $W$ is the number of operations performed by an application. $Q$ is the number of transferred bytes required during the program execution. Both $W$ and $Q$ define the operational intensity $I$ of applications as in Equation \ref{eq:PIWQ}. Characterizing applications by their intensity values is a conventional approach used in recent energy and performance modeling studies \cite{Choi2013, Choi2014, Ofenbeck:2014}.
\begin{equation} \label{eq:PIWQ}
	I= \frac{W}{Q}
\end{equation}
As the time required to perform one operation is different from the time required to transfer one byte of data, we introduce a parameter to the models: time ratio {$\alpha$} of transferring one byte of data to performing one arithmetic operation. Ratio {$\alpha$} is the property of an application on a specific platform and its value depends on the application. 
 
Since the time to access data and time to perform computation work can be overlapped, during a program execution, the core can be in one of the three states: performing computation, performing data transfer or performing both computation and data transfer in parallel. An application either has data transfer time longer than computation time or vice versa. Therefore, there are two models for the two cases. 
\begin{itemize}
\item If an application has data transfer time longer than computation time, it is memory-bound and follows Equation \ref{eq:PalbiWQ}. The execution can be modeled as two (composed) periods: one is when computation and data transfer are performed in parallel and the other is when only data transfer is performed. Fraction $\frac{W}{\alpha \times Q}$ represents the overlapped time of computation and data transfer. Fraction $\frac{\alpha \times Q-W}{\alpha \times Q}$ represents the remaining time for data transfer. 
\begin{equation} 
\label{eq:PalbiWQ} 
\begin{split}
	P&= P^{comp||data} \times \frac{W}{\alpha \times Q}+  P^{data} \times \frac{\alpha \times Q-W}{\alpha \times Q}
\end{split}
\end{equation}
\item If an application has computation time longer than data transfer time, it is compute-bound and follows Equation \ref{eq:PalleWQ}. The execution can be modeled as two periods: one is when computation and data transfer are performed in parallel and the other is when only computation is performed. Fraction $\frac{\alpha \times Q}{W}$ represents the overlapped time of computation and data transfer. Fraction $\frac{W-\alpha \times Q}{W}$ represents the remaining time for computation. 
\begin{equation} 
\label{eq:PalleWQ} 
\begin{split}
	P&= P^{comp||data} \times \frac{\alpha \times Q}{W} + P^{comp} \times \frac{W-\alpha \times Q}{W}
\end{split}
\end{equation}
\end{itemize}

After converting W and Q to I by using Equation \ref{eq:PIWQ}, the final models are simplified as Equation \ref{eq:PalbiI} and Equation \ref{eq:PalleI},
\begin{equation} 
\label{eq:PalbiI} 
\begin{split}
	P&= P^{comp||data} \times \frac{I}{\alpha}+  P^{data} \times \frac{\alpha-I}{\alpha}
\end{split}
\end{equation}
\begin{equation} 
\label{eq:PalleI} 
\begin{split}
	P&= P^{comp||data} \times \frac{\alpha}{I} + P^{comp} \times \frac{I-\alpha}{I}
\end{split}
\end{equation}
where $P^{data}$, $P^{comp}$ and $P^{comp||data}$ are explained below:
\paragraph{Data transfer power $P^{data}$} $P^{data}$ is the power consumed by the whole chip when only data transfer is performed. $P^{data}$ is computed by Equation \ref{eq:Pdata}. In Equation \ref{eq:Pdata}, 
%$P^{sta}$ is the static power; $P^{act}$ is the active power; $n$ is the number of active cores assigned to run the application;  
$m$ is the average number of cores accessing data in parallel during the application execution; contention power $P^{ctn}$ is the power overhead occurring when a core waits for accessing data because of the limited memory ports (or bandwidth) or cache size in the platform architecture. Therefore, $n-m$ is the average number of cores waiting for memory access during the application execution. 
\begin{equation} \label{eq:Pdata}
\begin{split}
	P^{data} &= P^{sta} + min(m,n) \times (P^{act}+ P^{LSU})\\
	&+ max(n-m, 0) \times P^{ctn} 
\end{split}
\end{equation}
\paragraph{Computation power $P^{comp}$} $P^{comp}$ is the power consumed by the whole chip when only computation is performed. $P^{comp}$ is computed by Equation \ref{eq:Pcomp}. Each core runs its arithmetic units (e.g. IAU, SAU, VAU) to perform computation work. There is no contention power due to no memory access. Therefore, all assigned cores are active and contribute to total power.
\begin{equation} 
\label{eq:Pcomp} 
\begin{split}
	P^{comp}&= P^{sta} + n \times (P^{act}+\sum_i{P^{dyn}_i(op)})
\end{split}
\end{equation}
\paragraph{Computation and data transfer power $P^{comp||data}$} $P^{comp||data}$ is the power consumed by the whole chip when computation and data transfer are performed in parallel. $P^{comp||data}$ is computed by Equation \ref{eq:Pcompdata}. In this case, there is contention power due to the data waiting. $P^{comp||data}$ is different from $P^{data}$ in the aspect that the active cores also run arithmetic units that contribute to total power as $\sum_i{P^{dyn}_i(op)}$.
\begin{equation} 
\label{eq:Pcompdata}
\begin{split}
	P^{comp||data} &= P^{sta} \\
	&+ min(m,n) \times (P^{act}+ P^{LSU}+\sum_i{P^{dyn}_i(op)}) \\
	&+ max(n-m, 0) \times P^{ctn}
\end{split}
\end{equation}
\subsection{Model Training and Validation}
\label{sec:Validation}
This section presents the experimental results of two sets of micro-benchmarks and three application kernels (i.e., {\it matmul}, SpMV and BFS) that are used for training and validating the models.
%This section presents the training and validation of the proposed models.
\subsubsection{Model Validation with Micro-benchmarks}
\label{sec:model-validation-micro}
Analyses of experimental results are performed based on two sets of micro-benchmarks: 26 micro-benchmarks for operation units called \emph{unit-suite} and 9 micro-benchmarks for different operational intensities called \emph{intensity-suite}. The measured power data is collected by executing each micro-benchmark with different numbers of cores (i.e., 1, 2, 4, and 8 cores).
\paragraph{Micro-benchmarks for Operation Units}
We assess the accuracy of the power model for operation units (Equation \ref{eq:Pfirst}) using data from \emph{unit-suite}. The model is trained with the power data collected when running \emph{unit-suite} with one and two cores. The power data collected when running \emph{unit-suite} with four and eight cores are used to validate the model. The micro-benchmarks of \emph{unit-suite} are listed in Table \ref{table:Micro-benchmarks}. 

We validate the model and plot its percentage errors in Figure \ref{fig:single-unit}. Percentage error is calculated as $PE=\frac{measurement - estimation}{measurement}$. 
Figure \ref{fig:single-unit} shows the percentage error of all three categories: one unit, two pipe-lined units and three pipe-lined units. The {\em absolute} percentage error is the absolute value of the percentage error. The model for operation units has the absolute percentage errors at most 8.5\%. These results prove that the model is applicable to micro-benchmarks using either a single (e.g., performing bit wise exclusive-OR on scalar unit: SauXor) or pipe-lined arithmetic units in parallel (e.g., performing Xor on scalar and integer units, in parallel with copying from scalar to scalar unit: SauXorCmuCpssIauXor). The model also shows the compositionality of the power consumption not only for multiple cores but also for multiple operation units within a core.

\begin{table*}
\caption{Micro-benchmarks for Operation Units}
\label{table:Micro-benchmarks}
\begin{center}
\footnotesize
\begin{tabular*}{15cm}{ll}
\hline\noalign{\smallskip}
Description & Micro-benchmark Name \\
\noalign{\smallskip}\hline\noalign{\smallskip}
 10 micro-benchmarks                 & SAUXOR, SAUMUL, IAUXOR, IAUMUL, VAUXOR, VAUMUL,\\
 using one unit (cf. Table 2)            & CMUCPSS, CMUCPIVR, LSULOAD, LSUSTORE\\ 
15 micro-benchmarks    &   SAUXOR-CMUCPSS, SAUXOR-CMUCPIVR, SAUXOR-IAUMUL,\\ 
 using two units  &   SAUXOR-IAUXOR, SAUXOR-VAUMUL, SAUXOR-VAUXOR,\\ 
      & SAUMUL-IAUXOR, IAUXOR-VAUXOR, IAUXOR-VAUMUL,\\ 
      & IAUXOR-CMUCPSS, LOAD-STORE, DUALLOAD, \\
      & DUALSTORE, SAUXOR-LOAD, SAUXOR-STORE   \\ 
1 micro-benchmarks & SAUXOR-IAUXOR-CMUCPSS \\ 
using three units & \\
\noalign{\smallskip}\hline\noalign{\smallskip}
\end{tabular*}
\end{center}
\end{table*}

\begin{figure}[!t] \centering
\small
\begin{tikzpicture}
\begin{axis}[
title=Percentage Errors of Micro-benchmarks for Operation Unit,
xlabel=Number of Cores,
ylabel=Percentage Error,
width=7cm, height=3.5cm,
%legend pos=outer north east,
legend style={at={(0.5,-0.5),font=\footnotesize},
anchor=north,legend columns=-1},
legend columns=3,
%symbolic x coords={0.25,0.5,1,2,4,8,16,32,64},
xtick=data,
xticklabels={1,2,4,8},
ytick={-10,-5,0,5,10},
yticklabel={\pgfmathprintnumber\tick\%}
]

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	main	SauMul	IauXor	IauMul 	VauXor	VauMul	CmuCpss	CmuCpivr	LSULoad	LSUStore
1	1.05	0.11	0.12	5.41	4.48	0.50	2.02	2.79	-3.23	-3.00
2	0.74	0.08	0.08	6.17	5.34	0.58	2.11	3.16	-4.42	-4.53
4	2.12	-0.34	-0.36	7.94	7.25	0.90	2.62	4.63	-4.38	-3.29
8	2.40	0.03	-0.44	8.53	8.51	1.79	3.23	5.00	-4.54	-7.00
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXor	main	IauXor	IauMul 	VauXor	VauMul	CmuCpss	CmuCpivr	LSULoad	LSUStore
1	1.05	0.11	0.12	5.41	4.48	0.50	2.02	2.79	-3.23	-3.00
2	0.74	0.08	0.08	6.17	5.34	0.58	2.11	3.16	-4.42	-4.53
4	2.12	-0.34	-0.36	7.94	7.25	0.90	2.62	4.63	-4.38	-3.29
8	2.40	0.03	-0.44	8.53	8.51	1.79	3.23	5.00	-4.54	-7.00
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXor	SauMul	main	IauMul 	VauXor	VauMul	CmuCpss	CmuCpivr	LSULoad	LSUStore
1	1.05	0.11	0.12	5.41	4.48	0.50	2.02	2.79	-3.23	-3.00
2	0.74	0.08	0.08	6.17	5.34	0.58	2.11	3.16	-4.42	-4.53
4	2.12	-0.34	-0.36	7.94	7.25	0.90	2.62	4.63	-4.38	-3.29
8	2.40	0.03	-0.44	8.53	8.51	1.79	3.23	5.00	-4.54	-7.00
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXor	SauMul	IauXor	main 	VauXor	VauMul	CmuCpss	CmuCpivr	LSULoad	LSUStore
1	1.05	0.11	0.12	5.41	4.48	0.50	2.02	2.79	-3.23	-3.00
2	0.74	0.08	0.08	6.17	5.34	0.58	2.11	3.16	-4.42	-4.53
4	2.12	-0.34	-0.36	7.94	7.25	0.90	2.62	4.63	-4.38	-3.29
8	2.40	0.03	-0.44	8.53	8.51	1.79	3.23	5.00	-4.54	-7.00
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXor	SauMul	IauXor	IauMul 	main	VauMul	CmuCpss	CmuCpivr	LSULoad	LSUStore
1	1.05	0.11	0.12	5.41	4.48	0.50	2.02	2.79	-3.23	-3.00
2	0.74	0.08	0.08	6.17	5.34	0.58	2.11	3.16	-4.42	-4.53
4	2.12	-0.34	-0.36	7.94	7.25	0.90	2.62	4.63	-4.38	-3.29
8	2.40	0.03	-0.44	8.53	8.51	1.79	3.23	5.00	-4.54	-7.00
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXor	SauMul	IauXor	IauMul 	VauXor	main	CmuCpss	CmuCpivr	LSULoad	LSUStore
1	1.05	0.11	0.12	5.41	4.48	0.50	2.02	2.79	-3.23	-3.00
2	0.74	0.08	0.08	6.17	5.34	0.58	2.11	3.16	-4.42	-4.53
4	2.12	-0.34	-0.36	7.94	7.25	0.90	2.62	4.63	-4.38	-3.29
8	2.40	0.03	-0.44	8.53	8.51	1.79	3.23	5.00	-4.54	-7.00
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXor	SauMul	IauXor	IauMul 	VauXor	VauMul	main	CmuCpivr	LSULoad	LSUStore
1	1.05	0.11	0.12	5.41	4.48	0.50	2.02	2.79	-3.23	-3.00
2	0.74	0.08	0.08	6.17	5.34	0.58	2.11	3.16	-4.42	-4.53
4	2.12	-0.34	-0.36	7.94	7.25	0.90	2.62	4.63	-4.38	-3.29
8	2.40	0.03	-0.44	8.53	8.51	1.79	3.23	5.00	-4.54	-7.00
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXor	SauMul	IauXor	IauMul 	VauXor	VauMul	CmuCpss	main	LSULoad	LSUStore
1	1.05	0.11	0.12	5.41	4.48	0.50	2.02	2.79	-3.23	-3.00
2	0.74	0.08	0.08	6.17	5.34	0.58	2.11	3.16	-4.42	-4.53
4	2.12	-0.34	-0.36	7.94	7.25	0.90	2.62	4.63	-4.38	-3.29
8	2.40	0.03	-0.44	8.53	8.51	1.79	3.23	5.00	-4.54	-7.00
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXor	SauMul	IauXor	IauMul 	VauXor	VauMul	CmuCpss	CmuCpivr	main	LSUStore
1	1.05	0.11	0.12	5.41	4.48	0.50	2.02	2.79	-3.23	-3.00
2	0.74	0.08	0.08	6.17	5.34	0.58	2.11	3.16	-4.42	-4.53
4	2.12	-0.34	-0.36	7.94	7.25	0.90	2.62	4.63	-4.38	-3.29
8	2.40	0.03	-0.44	8.53	8.51	1.79	3.23	5.00	-4.54	-7.00
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXor	SauMul	IauXor	IauMul 	VauXor	VauMul	CmuCpss	CmuCpivr	LSULoad	main
1	1.05	0.11	0.12	5.41	4.48	0.50	2.02	2.79	-3.23	-3.00
2	0.74	0.08	0.08	6.17	5.34	0.58	2.11	3.16	-4.42	-4.53
4	2.12	-0.34	-0.36	7.94	7.25	0.90	2.62	4.63	-4.38	-3.29
8	2.40	0.03	-0.44	8.53	8.51	1.79	3.23	5.00	-4.54	-7.00
};
%% combine with multiple-units
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	main	SauXorCmuCpivr	SauXorVauMul	SauXorVauXor	SauXorIauXor	SauXorIauMul 	IauXorVauMul	IauXorVauXor	SauMulIauXor 	IauXorCmuCpss	LoadStore	DualLoad	DualStore	SauXorLoad	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	main	SauXorVauMul	SauXorVauXor	SauXorIauXor	SauXorIauMul 	IauXorVauMul	IauXorVauXor	SauMulIauXor 	IauXorCmuCpss	LoadStore	DualLoad	DualStore	SauXorLoad	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	main	SauXorVauXor	SauXorIauXor	SauXorIauMul 	IauXorVauMul	IauXorVauXor	SauMulIauXor 	IauXorCmuCpss	LoadStore	DualLoad	DualStore	SauXorLoad	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	SauXorVauMul	main	SauXorIauXor	SauXorIauMul 	IauXorVauMul	IauXorVauXor	SauMulIauXor 	IauXorCmuCpss	LoadStore	DualLoad	DualStore	SauXorLoad	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	SauXorVauMul	SauXorVauXor	main	SauXorIauMul 	IauXorVauMul	IauXorVauXor	SauMulIauXor 	IauXorCmuCpss	LoadStore	DualLoad	DualStore	SauXorLoad	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	SauXorVauMul	SauXorVauXor	SauXorIauXor	main 	IauXorVauMul	IauXorVauXor	SauMulIauXor 	IauXorCmuCpss	LoadStore	DualLoad	DualStore	SauXorLoad	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	SauXorVauMul	SauXorVauXor	SauXorIauXor	SauXorIauMul 	main	IauXorVauXor	SauMulIauXor 	IauXorCmuCpss	LoadStore	DualLoad	DualStore	SauXorLoad	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	SauXorVauMul	SauXorVauXor	SauXorIauXor	SauXorIauMul 	IauXorVauMul	main	SauMulIauXor 	IauXorCmuCpss	LoadStore	DualLoad	DualStore	SauXorLoad	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	SauXorVauMul	SauXorVauXor	SauXorIauXor	SauXorIauMul 	IauXorVauMul	IauXorVauXor	main 	IauXorCmuCpss	LoadStore	DualLoad	DualStore	SauXorLoad	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	SauXorVauMul	SauXorVauXor	SauXorIauXor	SauXorIauMul 	IauXorVauMul	IauXorVauXor	SauMulIauXor 	main	LoadStore	DualLoad	DualStore	SauXorLoad	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	SauXorVauMul	SauXorVauXor	SauXorIauXor	SauXorIauMul 	IauXorVauMul	IauXorVauXor	SauMulIauXor 	IauXorCmuCpss	main	DualLoad	DualStore	SauXorLoad	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	SauXorVauMul	SauXorVauXor	SauXorIauXor	SauXorIauMul 	IauXorVauMul	IauXorVauXor	SauMulIauXor 	IauXorCmuCpss	LoadStore	main	DualStore	SauXorLoad	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	SauXorVauMul	SauXorVauXor	SauXorIauXor	SauXorIauMul 	IauXorVauMul	IauXorVauXor	SauMulIauXor 	IauXorCmuCpss	LoadStore	DualLoad	main	SauXorLoad	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	SauXorVauMul	SauXorVauXor	SauXorIauXor	SauXorIauMul 	IauXorVauMul	IauXorVauXor	SauMulIauXor 	IauXorCmuCpss	LoadStore	DualLoad	DualStore	main	SauXorStore	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	SauXorVauMul	SauXorVauXor	SauXorIauXor	SauXorIauMul 	IauXorVauMul	IauXorVauXor	SauMulIauXor 	IauXorCmuCpss	LoadStore	DualLoad	DualStore	SauXorLoad	main	SauXorCmuCpssIauXor
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x expr=\coordindex+1, y=main]
{
NumberOfCores	SauXorCmuCpss	SauXorCmuCpivr	SauXorVauMul	SauXorVauXor	SauXorIauXor	SauXorIauMul 	IauXorVauMul	IauXorVauXor	SauMulIauXor 	IauXorCmuCpss	LoadStore	DualLoad	DualStore	SauXorLoad	SauXorStore	main
1.00	0.10	0.88	-0.17	-2.29	-0.72	0.88	-0.17	-3.00	0.90	-0.73	0.08	1.43	1.28	0.09	2.17	3.05
2.00	0.07	0.59	0.13	-2.54	-0.48	0.58	-0.65	-3.44	0.60	-0.49	0.45	2.19	1.16	0.06	2.71	3.90
4.00	1.06	1.59	1.44	-2.20	-0.29	2.18	0.78	-2.72	1.63	-0.98	2.74	5.20	4.63	1.73	4.90	5.97
8.00	1.35	2.25	1.89	-1.85	0.21	2.39	1.30	-2.70	2.14	-0.36	2.93	6.15	5.38	2.19	5.73	6.06
};
%%
\legend{SauXor,SauMul,IauXor,IauMul,VauXor,VauMul,CmuCpss,CmuCpivr,LsuLoad,LsuStore, SauXorCmuCpss,SauXorCmuCpivr,SauXorVauMul,SauXorVauXor,SauXorIauXor,SauXorIauMul ,IauXorVauMul,IauXorVauXor,SauMulIauXor,IauXorCmuCpss,LoadStore	,DualLoad,DualStore,SauXorLoad,SauXorStore,SauXorCmuCpssIauXor} 
\end{axis}
\end{tikzpicture}
\caption{%The percentage errors of the model validation for \emph{unit-suite} for 10 one-unit micro-benchmark. The absolute percentage errors of micro-benchmarks for one-unit are at most 8.5\%.
The percentage errors of the model validation for \emph{unit-suite} for 26 micro-benchmark. The absolute percentage errors of unit-suite micro-benchmarks are at most 8.5\%.}
\label{fig:single-unit}
\end{figure}

%\comm{
%\input{diagram1}
%}
%%%%%%%%%%%%%%%%%%%%
%\comm{
%\input{diagram2}
%}
%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Micro-benchmarks for Application Intensities}
Since any application requires both computation and data movement, we design intensity-based micro-benchmarks which execute both arithmetic units (e.g., SAU) and two data transfer units (e.g., LSU0, LSU1) in a parallel manner. They are implemented with parallel instruction pipeline supported by the platform. In order to validate the RTHpower models, this \emph{intensity-suite} indicates different values of operation intensities (from 0.25 to 64). Operational intensity $I$ is retrieved from the assembly code by counting the number of arithmetic instructions and the number of load/store instructions. %%%%%Depending on whether computation time is longer than data transfer time, the power consumption follows either Equation \ref{eq:PalbiI} or Equation \ref{eq:PalleI} as described in Section \ref{sec:ModelEquation}.

In the models, there are platform-dependent parameters such as $\alpha$, $m$ and $P^{ctn}$. The parameter values for each application operational intensity are derived from experimental results by using Matlab function $lsqcurvefit$. For the application intensities from 0.25 to 1, $\alpha$ is found bigger than operational intensity $I$ meaning that data transfer time is longer than computation time. The estimated power model follows Equation \ref{eq:PalbiI}. For operational intensity from 2 to 64, $\alpha$ is less than $I$ meaning that data transfer time is less than computation time. The estimated power follows Equation \ref{eq:PalleI}.

We plot the percentage errors of the model fitting for intensity-based micro-benchmarks in Figure \ref{fig:Intensity-Deviation}. 
%%%%%The absolute percentage errors of intensity-based micro-benchmarks are at most 7\% for the operational intensity varying from 0.25 to 64.
%as shown in Table~\ref{table:TunableParameters}
\begin{figure}[!t] \centering
%\resizebox{1\columnwidth}{!}{ \includegraphics{figures/Intensity-Deviation.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=Percentage Errors of Intensity-based Micro-benchmarks,
xlabel=Operational Intensity,
ylabel=Percentage Error,
width=7cm, height=3.5cm,
%legend pos=outer north east,
legend style={at={(0.5,-0.5),font=\footnotesize},
anchor=north,legend columns=-1},
%symbolic x coords={0.25,0.5,1,2,4,8,16,32,64},
xtick={1,4,8,16,32,64},
%extra x tick style={xticklabel=\empty,grid=major},
ytick={-10,-5,0,5,10},
yticklabel={\pgfmathprintnumber\tick\%}
]

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=intensity, y=deviation]
{
intensity	1-core	deviation	4-cores	 6-cores	8-cores
0.25	15.15	3.46	-4.74	20.31	1.11
0.5	7.25	3.01	-3.69	13.16	0.84
1	7.75	2.56	-2.40	-7.04	0.79
2	1.37	1.78	-2.04	-2.01	0.50
4	2.72	1.44	-1.54	-1.74	0.37
8	-0.57	0.55	-0.59	35.18	0.10
16	-22.89	-1.65	5.14	89.87	-1.27
32	-22.66	0.64	4.16	98.80	-1.20
64	-18.98	7.13	-3.13	111.22	1.95
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=intensity, y=deviation]
{
intensity	1-core	2-cores	deviation	6-cores	8-cores
0.25	15.15	3.46	-4.74	20.31	1.11
0.5	7.25	3.01	-3.69	13.16	0.84
1	7.75	2.56	-2.40	-7.04	0.79
2	1.37	1.78	-2.04	-2.01	0.50
4	2.72	1.44	-1.54	-1.74	0.37
8	-0.57	0.55	-0.59	35.18	0.10
16	-22.89	-1.65	5.14	89.87	-1.27
32	-22.66	0.64	4.16	98.80	-1.20
64	-18.98	7.13	-3.13	111.22	1.95
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=intensity, y=deviation]
{
intensity	1-core	2-cores	4-cores	 6-cores	deviation
0.25	15.15	3.46	-4.74	20.31	1.11
0.5	7.25	3.01	-3.69	13.16	0.84
1	7.75	2.56	-2.40	-7.04	0.79
2	1.37	1.78	-2.04	-2.01	0.50
4	2.72	1.44	-1.54	-1.74	0.37
8	-0.57	0.55	-0.59	35.18	0.10
16	-22.89	-1.65	5.14	89.87	-1.27
32	-22.66	0.64	4.16	98.80	-1.20
64	-18.98	7.13	-3.13	111.22	1.95
};
\legend{2-cores, 4-cores, 8-cores} 
\end{axis}
\end{tikzpicture}
\caption{The absolute percentage errors of RTHpower model fitting for \emph{intensity-suite} (operational intensity $I$ from 0.25 to 64) are at most 7\%.}
\label{fig:Intensity-Deviation}
\end{figure}
In order to obtain a  full range of estimated power with any values of intensities and numbers of cores, a fuzzy logic approach, namely Takagi Sugeno Kang (TSK) mechanism \cite{6313399}, is applied to the RTHpower models. Each intensity has a parameter set, including $\alpha$, $P^{ctn}$ and $m$. Based on the RTHpower models, each parameter set provides an individual function to estimate the power of an application based on its intensity value and a number of cores. 

The TSK mechanism considers the individual functions as membership functions and combines them into a general function that can be used for any input (i.e., intensity $I$ and number of cores $n$). The membership function of the fuzzy sets are triangular. After implemented the approach using Matlab Fuzzy Logic toolbox, the full range of estimated power is obtained and presented in Figure \ref{fig:TSKEstimation}. It is observed that when intensity value increases, the power-up (i.e., the power consumption ratio of the application executed with $n$ cores to the application executed with 1 core) is also increased. When intensity increases, the platform total power if running an application with 1 core slightly increases while the platform total power if running the application with $n$ cores increases more significant. The small dip in the diagram is due to the switch from Equation \ref{eq:PalbiI} to Equation \ref{eq:PalleI} at the intensity $I=2$.
\begin{figure}[!t] \centering
\resizebox{0.9\columnwidth}{!}{ \includegraphics{figures/Power_range.png}}
\caption{The power range of varied intensities and numbers of cores from RTHpower models. The dots in the figure represent measurement data. The model switches from Equation \ref{eq:PalbiI} to Equation \ref{eq:PalleI} at the intensity $I=2$}
\label{fig:TSKEstimation}
\end{figure}
%For the benchmarks which have the operational intensity that is different from the available intensity in Table \ref{table:TunableParameters}, the general estimation are combined with a fuzzy logic mechanism, namely Takagi Sugeno Kang (TSK) mechanism \cite{Sugeno:1985}. are blend the provided functions based on an antecedent variable (in our case the intensity) to calculate the output. Each combination of parameters provide a function to estimate the power of the benchmark based on a corresponding intensity value.  This mechanism combines individual functions into a general function that can be used for any input values (intensity and number of cores). In this paper, the triangular membership functions are used.
\comm{%%%%%%%%%%%%%%
\begin{table}
\caption{Model parameters values}
\label{table:TunableParameters}
\begin{center}
\begin{tabular}{llll}
\hline\noalign{\smallskip}
Intensity 	& $m$ & $P^{ctn}$ & $\alpha$ 	\\
\noalign{\smallskip}\hline\noalign{\smallskip}
0.25	&0.72	&9.89	&0.93	\\
0.5	&0.57	&15.64	&2.27	\\
1	&0.57	&18.39	&1.87	\\
2	&0.80	&7.77	&0.94	\\
4	&0.83	&0.97	&1.69	\\
8	&1.05	&0.9	&2.43	\\
16	&0.001	&0.03	&2.03	\\
32	&0.001	&0.05	&2.15	\\
64	&3.17	&0.001	&2.62   \\
\noalign{\smallskip}\hline\noalign{\smallskip}
\end{tabular}
\end{center}
\end{table}
}%%%%%%%%%%%%%%%

\subsubsection{Model Validation with Application Kernels}
The following application kernels have been chosen to implement and validate the RTHpower models on Myriad1: {\it matmul} (a computation-intensive kernel), SpMV (a kernel with dynamic access patterns), and BFS (a data-intensive kernel) \cite{6114175}. The three kernels are able to cover the two dimensions of operational intensity and speed-up as shown in Figure \ref{fig:App-Cate}.
%Because the operational intensity and performance scalability are the important factors in RTHpower models and RTH framework (cf. Section \ref{sec:Framework}), the chosen kernels have varied levels of intensity and scalability values as in Figure \ref{fig:App-Cate}.
 
{\it Matmul} is proved to have high intensity and scalability \cite{Ofenbeck:2014}. SpMV has low operational intensity and high speed-up due to its parallel scalability \cite{William2007}. BFS, on the other hand, has low operational intensity and saturated low scalability \cite{Cook:2013}. Since the available benchmark suites in literature are not executable on Myriad1 platform, the three mentioned kernels have been implemented by the authors using the Movidius Development Kit for Myriad1. As the RTHpower models will be used to predict whether the RTH strategy is an energy efficient approach for a given application, we focus mainly on two settings: the 8-core setting representing the RTH strategy (i.e., using all available cores of Myriad1) and the 1-core setting  representing the other extreme (i.e., using a minimum number of cores).
\begin{figure}[!t] \centering
\resizebox{0.6\columnwidth}{!}{ \includegraphics{figures/App-Cate.png}}
\caption{Application Categories}
\label{fig:App-Cate}
\end{figure}
\paragraph{Dense Matrix Multiplication}
{\it Matmul} has been implemented on Myriad1 by using both C and assembly languages. The {\it matmul} algorithm computes matrix C based on two input matrices A and B $C=A \times B$. All three matrices in this benchmarks are stored in DDR RAM. Matrix elements are stored with float type equivalent to four bytes. The number of operations and accessed data are calculated based on matrix size $n$ as: $W=2\times n^3$ and $Q=16\times n^2$  \cite{Ofenbeck:2014}. Intensity of {\it matmul} is also varied with matrix size as: $I = \frac{W}{Q} = \frac{n}{8}$. %In our experiments, we measured power consumption of matmul with size $128 \times 128$ to $1024 \times 1024$.
The experiments are conducted until matrix size 1024x1024, the largest size that Myriad1 RAM memory can accommodate. %Figure \ref{fig:MatmulDeviation} shows that the percentage error of {\it matmul} estimated power compared to measured power is -25\% on average for 1 core and 12\% on average for 8 cores.
 
We observe that operational intensity is not enough to capture other factors affecting power consumption such as the communication patterns and potential performance/power overheads due to the implementation. E.g., although a sequential version and a parallel version of a {\it matmul} algorithm have the same intensity, it is obvious that they have different communication pattern (intuitively, the sequential version does not have communication between cores). Since different parallel versions for different number of cores have different communication patterns (e.g., sequential version vs. 8-core version), ignoring the mentioned factors contributes to the percentage errors. Therefore, we apply online-learning approaches, which are widely used to learn characteristics of an application while it is running \cite{Mishra:2015}, to RTHpower models. Applying the online-learning approach results in Equation \ref{eq:Pimp1} and Equation \ref{eq:Pimp2}, where $\beta$ is computed by using few sample executions in Equation \ref{eq:beta}.  
\begin{equation} 
\label{eq:Pimp1} 
\begin{split}
	P_{improved}= (P^{comp||data} \times \frac{I}{\alpha}+  P^{data} \times \frac{\alpha-I}{\alpha}) \times \beta
\end{split} 
\end{equation}
\begin{equation} 
\label{eq:Pimp2} 
\begin{split}
	P_{improved}= (P^{comp||data} \times \frac{\alpha}{I} + P^{comp} \times \frac{I-\alpha}{I})\times \beta
\end{split} 
\end{equation}
\begin{equation} 
\label{eq:beta} 
\begin{split}
\beta = \frac{1}{1 + \overline{PE}}.
\end{split} 
\end{equation}

Note that parameter $\beta$ for each sequential/parallel version (e.g., 1-core version or 8-core version) is fixed across problem sizes and therefore it can be obtained during kernel installation and then saved as meta-data for each version in practice. E.g., the average of matmul percentage errors is 28\% for 1-core and 13\% for 8-cores, therefore, the $\beta$ values of {\it matmul} are $\frac{1}{1 - 28\%}$ for 1-core and $\frac{1}{1 + 13\%}$ for 8-cores. $\beta$ is computed by using data from sample executions with two matrix sizes (i.e., 128x128, and 512x512). The test set to validate the model is data from executions with four matrix sizes (i.e., 128x128, 256x256, 512x512, and 1024x1024). The absolute percentage errors are at most 12\% as shown in Figure \ref{fig:MatmulDeviation}.
%{\it Matmul} has highest modeling errors among three validated application kernels since {\it matmul} has varied intensity values on different matrix sizes.
\begin{figure}[!t] \centering
\small
\begin{tikzpicture}
\begin{axis}[
title=Model Percentage Errors of Dense Matrix Multiplication,
xlabel=Matrix Size,
ylabel=Percentage Error,
width=7cm, height=4cm,
%legend pos= outer north east,
legend style={at={(0.5,-0.5),font=\footnotesize},
anchor=north,legend columns=-1},
legend columns=2,
symbolic x coords={
128x128,
256x256,
512x512,
1024x1024,
},
x tick label style={rotate=30,anchor=east},
xticklabel style = {xshift=-0.10cm},
ytick={-30,-20,-10,0,10,20},
yticklabel={\pgfmathprintnumber\tick\%}
]
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	1-core 8-cores deviation 8-cores-after-improved
128x128	-31.34	2.29	-4.53	-10.04
256x256	-29.06	14.78	-1.17	1.94
512x512	-25.13	22.82	4.15	8.36
1024x1024	-17.78	20.72	12.71	6.76
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	1-core 8-cores 1-core-after-improved deviation
128x128	-31.34	2.29	-4.53	-10.04
256x256	-29.06	14.78	-1.17	1.94
512x512	-25.13	22.82	4.15	8.36
1024x1024	-17.78	20.72	12.71	6.76
};
%\legend{1-core-original,8-cores-original,1-core-improved,8-cores-improved} 
\legend{1-core,8-cores}
\end{axis}
\end{tikzpicture}
\caption{Absolute percentage errors of estimated power from measured power of {\it matmul}. After applying the online-learning approach, the absolute percentage errors of {\it matmul} are at most 12\%.}
\label{fig:MatmulDeviation}
\end{figure}
\comm{
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	deviation 8-cores 1-core-after-improved 8-cores-after-improved
128x128	-31.34	2.29	-4.53	-10.04
256x256	-29.06	14.78	-1.17	1.94
512x512	-25.13	22.82	4.15	8.36
1024x1024	-17.78	20.72	12.71	6.76
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	1-core deviation 1-core after improved 8-cores after improved
128x128	-31.34	2.29	-4.53	-10.04
256x256	-29.06	14.78	-1.17	1.94
512x512	-25.13	22.82	4.15	8.36
1024x1024	-17.78	20.72	12.71	6.76
};
}

\paragraph{Sparse Matrix Vector Multiplication}
SpMV implementation on Myriad1 is written in C language. All input matrix and vector of this benchmark reside in DDR RAM. This implementation uses the common data layout of SpMV which is compressed sparse row (csr) format \cite{Saad:2003}. There is no random generator supported in the RISC core so a 5 non-zero elements per row is fixed in all experiments. 
Each element of matrix and vector is stored with float type of four bytes. %Since the whole matrix is stored before performing computation in CSR format, the experiments are conducted until matrix size $2048x2048$ which is the largest that RAM memory can accommodate. 
From our implementation analysis, the number of operations and accessed data are proportional to the size of a matrix dimension $n$ as: $W=5 \times 2\times n$ and $Q=5 \times 2 \times 4 \times n$. Operational intensity of SpMV  therefore, does not depend on matrix size and is a fixed value: $I = \frac{W}{Q}= 0.25$.

Figure \ref{fig:SpMVDeviation} shows the percentage error of SpMV estimated power using Equation \ref{eq:Pimp1} and \ref{eq:Pimp2} compared to measured power. The $\beta$ values for 1-core and 8-core versions of SpMV are computed from executions with three matrix sizes (i.e., 32x32, 128x128, and 512x512) as $\frac{1}{1 + 14\%}$ and $\frac{1}{1 - 8\%}$, respectively. The model is validated with test data from executions with six matrix sizes (i.e., 32x32, 64x64, 128x128, 256x256, 512x512, and 1024x1024) and has the absolute percentage errors at most 4\% as shown in Figure \ref{fig:SpMVDeviation}. 
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{figures/SpMVDeviation.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=Model Percentage Errors of Sparse Matrix Vector Multiplication,
xlabel=Matrix Size,
ylabel=Percentage Error,
width=7cm, height=4cm,
%legend pos= outer north east,
legend style={at={(0.5,-0.5),font=\footnotesize},
anchor=north,legend columns=-1},
legend columns=2,
symbolic x coords={32x32,
64x64,
128x128,
256x256,
512x512,
1024x1024,
},
x tick label style={rotate=35,anchor=east},
xticklabel style = {xshift=-0.10cm},
ytick={-4,-2,0,2,4},
yticklabel={\pgfmathprintnumber\tick\%}
]

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	1-core 8-cores deviation 8-cores-after-improved
32x32	14.19	-6.25	0.28	3.32
64x64	14.19	-8.74	0.28	0.68
128x128	14.19	-9.93	0.28	-0.63
256x256	15.15	-10.32	1.11	-1.07
512x512	13.25	-7.92	-0.55	1.56
1024x1024	13.25	-6.25	-0.55	3.32

};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	1-core 8-cores 1-core-after-improved deviation
32x32	14.19	-6.25	0.28	3.32
64x64	14.19	-8.74	0.28	0.68
128x128	14.19	-9.93	0.28	-0.63
256x256	15.15	-10.32	1.11	-1.07
512x512	13.25	-7.92	-0.55	1.56
1024x1024	13.25	-6.25	-0.55	3.32
};
%\legend{1-core-original,8-cores-original,1-core-improved,8-cores-improved} 
\legend{1-core,8-cores} 
\end{axis}
\end{tikzpicture}
\caption{Absolute percentage errors of estimated power from measured power of SpMV. After applying the online-learning approach, the absolute percentage errors of SpMV are at most 4\%.}
\label{fig:SpMVDeviation}
\end{figure}
\comm{
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	deviation 8-cores 1-core-after-improved 8-core-after-improved
32x32	14.19	-6.25	0.28	3.32
64x64	14.19	-8.74	0.28	0.68
128x128	14.19	-9.93	0.28	-0.63
256x256	15.15	-10.32	1.11	-1.07
512x512	13.25	-7.92	-0.55	1.56
1024x1024	13.25	-6.25	-0.55	3.32
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=size, y=deviation]
{
size	1-core deviation 1-core-after-improved 8-core-after-improved
32x32	14.19	-6.25	0.28	3.32
64x64	14.19	-8.74	0.28	0.68
128x128	14.19	-9.93	0.28	-0.63
256x256	15.15	-10.32	1.11	-1.07
512x512	13.25	-7.92	-0.55	1.56
1024x1024	13.25	-6.25	-0.55	3.32
};
}
\paragraph{Breadth First Search}
We also implemented BFS-a data-intensive Graph500 kernel, on Myriad1. BFS is the graph kernel to explore the vertices and edges of a directed graph from a starting vertex. We use the implementation of current Graph500 benchmark (omp-csr) and port it to Myriad1. The output BFS graphs after running BFS implementation on Myriad1 are verified by the verification step of original Graph500 code to ensure that the output graphs are correct.

The size of a graph is defined by its scale and edgefactor. In our experiments, we mostly use the default edgefactor of 16 from the Graph500 so that each vertex of the graph has $16$ edges in average. The graph scales are varied from 14 to 17 and the graphs has from $2^{14}$ to $2^{17}$ vertices. It is noted that graph scale 17 is the largest scale that the DDR RAM of Myriad1 can accommodate. From the implementation analysis, the operational intensity of BFS is a fixed value: $I = \frac{W}{Q} = 0.257$ and does not depend on edgefactor or scale. 

Figure \ref{fig:BFSDeviation} shows the percentage error of BFS estimated power using Equation \ref{eq:Pimp1} and \ref{eq:Pimp2} compared to measured power. 
The $\beta$ values for 1-core and 8-core versions of BFS are computed from executions with two graph scales (i.e., 14 and 16) as $\frac{1}{1 + 9\%}$ and $\frac{1}{1 - 18\%}$, respectively. The test set to validate the model is data from executions with four graph scales (i.e., 14-17) and has the absolute percentage errors at most 3\% as shown in Figure \ref{fig:BFSDeviation}.
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{figures/BFSDeviation.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=Model Percentage Errors of Breadth First Search,
xlabel=Graph Scale,
ylabel=Percentage Error,
width=7cm, height=4cm,
legend style={at={(0.5,-0.5),font=\footnotesize},
anchor=north,legend columns=-1},
legend columns=2,
%legend pos= outer north east,
%x tick label style={rotate=45,anchor=east},
symbolic x coords={14,15,16,17},
ytick={-4,-2,0,2,4},
yticklabel={\pgfmathprintnumber\tick\%},
]

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=scale, y=deviation]
{
scale	deviation	8-cores-after	1-core-before	8-cores-before
14	0.00	0.79	8.81	-17.79
15	-2.33	-1.18	6.28	-19.40
16	0.00	-0.79	8.81	-19.08
17	0.00	-1.18	8.81	-19.40

};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=scale, y=deviation]
{
scale	1-core-after	deviation	1-core-before	8-cores-before
14	0.00	0.79	8.81	-17.79
15	-2.33	-1.18	6.28	-19.40
16	0.00	-0.79	8.81	-19.08
17	0.00	-1.18	8.81	-19.40
};
%\legend{1-core-original,8-cores-original,1-core-improved,8-cores-improved} 
\legend{1-core,8-cores}
\end{axis}
\end{tikzpicture}
\caption{Absolute percentage errors of estimated power from measured power of BFS. After applying the online-learning approach, the absolute percentage errors are at most 3\%.}
\label{fig:BFSDeviation}
\end{figure}
\comm{
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=scale, y=deviation]
{
scale	1-core-after	8-core-after	deviation	8-cores-before
14	0.00	0.79	8.81	-17.79
15	-2.33	-1.18	6.28	-19.40
16	0.00	-0.79	8.81	-19.08
17	0.00	-1.18	8.81	-19.40
};
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=scale, y=deviation]
{
scale	1-core-after	8-cores-after	1-core-before	deviation
14	0.00	0.79	8.81	-17.79
15	-2.33	-1.18	6.28	-19.40
16	0.00	-0.79	8.81	-19.08
17	0.00	-1.18	8.81	-19.40
};
}
Both SpMV and BFS in our experiments have lower modeling errors than {\it matmul} since they have a fixed intensity value on different matrix sizes.
\subsection{Race-to-halt Prediction Framework}
\label{sec:Framework} 
%RTH, a popular energy-saving strategy in high performance computing platforms, might not be true for ULP platforms due to their low static power. 
With RTHpower models, we want to identify whether RTH strategy is energy-efficient for an application and how many cores the system should use to run an application to achieve the least energy consumption. In order to answer the questions, we need to consider the speed-up and power-up of an application on a specific platform. 

From Amdahl's Law \cite{4563876} the theoretical maximum speed-up of an application running on a multicore system is derived as Equation \ref{eq:Amdahl-law}, where $p$ denotes the fraction of the application that can be parallelized and $n$ is the number of cores:
\begin{equation} 
\label{eq:Amdahl-law} 
	\mbox{\it speed-up} \leq \frac{1}{(1-p)+ \frac{p}{n}}
\end{equation}
\subsubsection{Framework Description}
The purpose of this framework is to identify when to and when not to use RTH for a given application. The two required inputs for making decision are power-up and speed-up of the application executed with $n$ cores, where $n$ is the maximum number of cores. 
\begin{itemize}
\item Step 1: Identify meta-data, including speed-up and operational intensity, of a given application by one of the three main approaches listed: i) doing theoretical analysis to find the amount of computation work $W$, data transfer $Q$ and operational intensity $I$ as well as identify the maximum speed-up of a given application; ii) executing the application on a targeted platform (e.g., Myriad1) to measure its speed-up and extract its operational intensity $I$; iii) using profiling tools \cite{Liu2014} to extract the number of operations $W$ and the amount of data transferred $Q$ as well as the speed-up of an application on a common platform (e.g., Intel platform).
\item Step 2: Compute power consumption of an application running with one core and with a maximum number of cores by the RTHpower models. Note that the RTHpower models are able to estimate power consumption for any number of cores by changing parameter $n$ in the models. For verifying RTH strategy, we only need to apply the model for a single core and all cores. 
\item Step 3: Compare the energy consumption of the application between using one core and using a maximum number of cores to identify whether running a maximum number of cores is the most energy-efficient.
\end{itemize}

The framework is designed for kernels of libraries that will be executed several times. A kernel need to pre-run twice (i.e., with one core and with a maximum number of core) to find the speed-up while power-up is predicted by the RTHpower models. After deciding whether to use RTH for a kernel, the decision is beneficial for the remaining executions of the kernel.
\subsubsection{Framework Validation}
The framework is validated with three micro-benchmarks and three application kernels. In this validation, the values of operational intensity $I$ are extracted from theoretical analysis of the implementations and speed-up is identified by executing the micro-benchmarks or application kernels with different numbers of cores.
\paragraph{Race-to-halt for Micro-benchmarks}
% For intensity $I=0.25$, we create three micro-benchmarks: a program with 60\% parallel code, a program with 100\% parallel code and a small-size micro-benchmarks which has high overhead. If the speed-up is bigger than the power ratio (namely, power-up), RTH is an energy-saving strategy. If the speed-up is less than the power-up, running with the maximum number of cores will consume more energy and race-to-halt is no longer applicable for saving energy. Figure \ref{fig:Micro-Speed-up} shows the power-up  of a program running $n$ cores to the program running one core for intensity 0.25. speed-up for all three reported micro-benchmarks is less than the power-up over different numbers of cores. This explains why RTH is not applicable for these three programs.
We first validate the framework with micro-benchmarks. In this validation, we measure the power-up and speed-up of three micro-benchmarks: one with 60\% parallel code, one with 100\% parallel code and a small-size micro-benchmarks which has high overhead. All three micro-benchmarks have operational intensity $I=0.25$. Namely, in the micro-benchmarks, each SauXor instruction is followed by a LsuLoad instruction which loads 4 bytes.

All three micro-benchmarks have the same assembly code wrapped inside a loop. The number of iterations to repeat the code are the difference among them. 
We run the micro-benchmarks on one core for 1 000 000 times. If the micro-benchmark has 100\% parallel code, running it on $n$ core requires each core performing $\frac{1}{n}$ of the amount of work (e.g., if performing the micro-benchmark on 8 cores, each core needs to run 125 000 times). Similarly, if the micro-benchmark has a parallel fraction of 60\%, then running the program on $n$ cores requires each core to perform $(1-0.6)+(\frac{0.6}{n})$ of the amount of work (e.g.,if performing the micro-benchmark on 8 cores, each core needs to run 475 000 times). For small-size micro-benchmark, the code is executed 8 times with 1 core and once with 8 cores. Since the amount of computation is small, the relative overhead of initializing the platform and executing the small-size micro-benchmark is high. 

Figure \ref{fig:Micro-Speed-up} shows that the power-up of running $n$ cores to the program running 1 core varies from 1 (1 core) to 1.71 (8 cores) for operational intensity $I=0.25$. If the speed-up is bigger than the power-up, RTH is an energy-saving strategy. If the speed-up is less than the power-up, running the program with the maximum number of cores consumes more energy than running it with 1 core. Note that when this happens, assigning one core to run the program is more energy-efficient and race-to-halt is no longer applicable for saving energy. For all three micro-benchmarks in this validation, the speed-up is identified by running them over different numbers of cores.
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{figures/Micro-Speed-up.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=Speed-up and Power-up of Micro-benchmarks,
xlabel=Number of Cores,
%ylabel=Energy-saving Percentage,
width=7cm, height=3.5cm,
legend style={at={(0.5,-0.5),font=\footnotesize},
anchor=north,legend columns=-1},
legend columns=2,
xtick={1, 2, 4, 8},
%symbolic x coords={1,2,4,8},
%ytick={-20,-10,0,10,20},
]

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=cores, y=powerscalability]
{
cores	powerscalability
1	1
2	1.193277311
4	1.470588235
8	1.714285714
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=cores, y=speedup]
{
cores speedup 
1	1
2	0.910371319
4	1.142168675
8	1.102325581
};


\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=cores, y=speedup]
{
cores speedup 
1	1
2	0.649908592
4	0.424985057
8	0.296806512
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[x=cores, y=speedup]
{
cores speedup 
1	1
2	0.75
4	0.75
8	0.375
};

\legend{Power-up, Speed-up-100\%-parallel, Speed-up-60\%-parallel, Speed-up-small-size} 
\end{axis}
\end{tikzpicture}
\caption{Speed-up and power-up of micro-benchmarks with operational intensity $I=0.25$. All three reported micro-benchmarks have speed-up less than platform power-up.}
\label{fig:Micro-Speed-up}
\end{figure}
The energy consumption of the three micro-benchmarks is shown in Figure \ref{fig:Micro-Energy}. All three micro-benchmarks achieve the least energy consumption when executed with one core, from both measured and estimated data. The model estimation and actual measurement show that RTH is not applicable to the three micro-benchmarks.
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{figures/Micro-Energy.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=Energy Consumption of Micro-benchmarks,
xlabel=Number of Cores,
ylabel=Energy (mJ),
width=7cm, height=3.5cm,
legend style={at={(0.5,-0.5),font=\footnotesize},
anchor=north,legend columns=-1},
legend columns=2,
%symbolic x coords={1, 2, 4, 8},
xtick={1, 2, 4, 8},
%x tick label style={rotate=35,anchor=east},
%ytick={-20,-10,0,10,20},
%yticklabel={\pgfmathprintnumber\tick\%}
]

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[]
{
x	y
1	169.218
2	221.804
4	217.875
8	263.16

};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[]
{
x	y
1	194.8528068
2	229.4848075
4	207.5381265
8	266.0719045
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[]
{
x	y
1	169.218
2	310.696
4	585.55
8	977.364
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[]
{
x	y
1	194.8528068
2	321.4550312
4	557.7691334
8	988.1786779
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[]
{
x	y
1	342
2	500
4	600
8	1616
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[]
{
x	y
1	357
2	568
4	700
8	1632
};

\legend{100\%-parallel-measurement,100\%-parallel-estimation,60\%-parallel-measurement,60\%-parallel-estimation, small-size-measurement,small-size-estimation} 
\end{axis}
\end{tikzpicture}
\caption{Energy consumption of micro-benchmarks with operational intensity $I=0.25$.
For all three reported micro-benchmarks, the programs executed with 1 core consume the least energy, compared to 2, 4, 8 cores, from both measured data and estimated data.}
\label{fig:Micro-Energy}
\end{figure}
\paragraph{Race-to-halt for Dense Matrix Multiplication}
The {\it matmul} application has increasing values of operational intensity over input sizes and its speed-up is higher than its power-up on Myriad1. 
Therefore, running {\it matmul} with the 8 cores is more energy-efficient than running it with one core. Figure \ref{fig:Matmul-RTH} shows how many percentages of energy-saving if executing {\it matmul} with 8 cores instead of 1 core, from both measured and estimated data. The energy saving percentage is computed based on the energy gap of running 1 core and 8 cores divided by energy consumed by running 1 core as in Equation \ref{eq:ES}.
\begin{equation} 
\label{eq:ES} 
	 ES = \frac{E^{1core} - E^{8cores}}{E^{1core}}
\end{equation}
The framework can predict that RTH should be applied to {\it matmul} over different matrix sizes. By using RTH for {\it matmul}, we can save from 20\% to 61\% of {\it matmul} energy consumption. RTH is a good strategy for {\it matmul}. We observe that the energy saving reduces when matrix size increases due to the decrease of speed-up from size 128x128. The reason is that a matrix size bigger than 128x128 makes the data set no longer fit in the last level cache (or L2 cache of 64KB) and thereby lowers performance (in flops).  
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{figures/SpMV-RTH.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=Matmul Energy-saving by Race-to-halt,
xlabel=Matrix Size,
ylabel=Energy-saving Percentage,
width=6cm, height=4cm,
legend style={at={(0.5,-0.5),font=\footnotesize},
anchor=north,legend columns=-1},
symbolic x coords={
128x128,
256x256,
512x512,
},
x tick label style={rotate=35,anchor=east},
xticklabel style = {xshift=-0.10cm},
%ytick={-20,-10,0,10,20},
yticklabel={\pgfmathprintnumber\tick\%}
]
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[y error=error]
{
x y error
128x128	60.20	0.00
256x256	30.32	0.52
512x512	26.28	0.03
%1024x1024	-288.77	-18.91

};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[y error=error]
{
x y error
128x128	62.20	0.00
256x256	28.11	0.62
512x512	22.89	0.04
%1024x1024	-263.95%	-19.64%
};

\legend{Measurement, Model Estimation} 
\end{axis}
\end{tikzpicture}
\caption{{\it Matmul} energy-saving by Race-to-halt. This diagram shows how many percentages of energy-saving if execute {\it matmul} with 8 cores instead of 1 core. Since the energy-saving percentage is positive over different matrix sizes, RTH is a energy-saving strategy for {\it matmul}. Energy-saving percentage from model estimation for {\it matmul} has standard deviation less than 3\%.}
\label{fig:Matmul-RTH}
\end{figure}
\paragraph{Race-to-halt for Sparse Matrix Vector Multiplication}
SpMV has a fixed value of operational intensity over input sizes. From the RTHpower models as well as measurement data, the power-up of SpMV is relatively constant. However, SpMV has speed-up higher than its power-up. 
Therefore, running SpMV with the maximum number of cores is more energy-efficient than running it with one core. Figure \ref{fig:SpMV-RTH} shows how many percentages of energy-saving if executing SpMV with 8 cores instead of 1 core, from both measured and estimated data. The framework can predict that RTH should be applied to SpMV over different matrix sizes. By using RTH for SpMV, we can save from 45\% to 59\% of SpMV energy consumption. RTH is a good strategy for SpMV. The energy saving increases from size 32x32 to 128x128 since the data fits in L1 cache. 
%From size 256x256 to 1024x1024, the data fits to L2 cache. 
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{figures/SpMV-RTH.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=SpMV Energy-saving by Race-to-halt,
xlabel=Matrix Size,
ylabel=Energy-saving Percentage,
width=8cm, height=4cm,
legend style={at={(0.5,-0.5),font=\footnotesize},
anchor=north,legend columns=-1},
symbolic x coords={32x32,
64x64,
128x128,
256x256,
512x512,
1024x1024,
%2048x2048,
},
x tick label style={rotate=35,anchor=east},
xticklabel style = {xshift=-0.10cm},
%ytick={-20,-10,0,10,20},
yticklabel={\pgfmathprintnumber\tick\%}
]
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[y error=error]
{
x y error
32x32	46.46	0.00
64x64	53.76	0.98
128x128	59.28	0.55
256x256	58.14	3.00
512x512	55.46	1.66
1024x1024	49.06	1.34
%2048x2048	59.54	0.56
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[y error=error]
{
x y error
32x32	44.78	0.00
64x64	53.57	0.97
128x128	59.65	0.56
256x256	59.05	3.04
512x512	54.50	1.63
1024x1024	47.02	1.29

};

\legend{Measurement, Model Estimation} 
\end{axis}
\end{tikzpicture}
\caption{SpMV Energy-saving by Race-to-halt. This diagram shows how many percentages of energy-saving if execute SpMV with 8 cores instead of 1 core. Since the energy-saving percentage is positive over different matrix sizes, RTH is a energy-saving strategy for SpMV.}
\label{fig:SpMV-RTH}
\end{figure}
\paragraph{Race-to-halt for Breadth First Search}
In our set of application kernels implemented on Myriad1, 
BFS is the application kernel able to prove that running with a
maximum number of cores does not always give the least energy consumption. From both measured data and estimated data, the total energy consumed by running with one core is less than the total energy by running with 8 cores at scale 16 and 17. There are negative values of -5\% and -3\% in Figure \ref{fig:BFS-RTH} if running BFS with 8 cores instead of 1 cores at scale 16 and 17, respectively. The RTHpower models can predict when to apply RTH for different scales. 
%The models show that RTH should be applied on scale 14 and 15 while it should not be applied on scale 16 and 17. 

The result can be explained by the relation between BFS power-up and speed-up. Since BFS has a fixed value of operational intensities across graph scale, from RTHpower models (cf. Equation \ref{eq:Pimp1} and \ref{eq:Pimp2}), it is understood that BFS power consumption does not depend on graph scales and its power-up is a fixed value. From the measurement results, we also observe that BFS power-scalability is relatively constant over the graph scales. However, BFS speed-up in our experiments decreases when scale increases. The reason is that with the same graph degree, when scale increases, the graph becomes more sparse and disconnected. Compared to the Graph500 implementation, BFS search on Myriad1 are performed from a chosen subset of source nodes. The speed-up then, becomes less than power-up at scale 16 and 17. Therefore, running BFS with 8 cores at bigger graph scales (i.e., 16 and 17 in our experiments) consumes more energy than running BFS with one core.
\begin{figure}[!t] \centering
%\resizebox{0.8\columnwidth}{!}{ \includegraphics{figures/BFS-RTH.png}}
\small
\begin{tikzpicture}
\begin{axis}[
title=BFS Energy-saving by Race-to-halt,
xlabel=Graph Scale,
ylabel=Energy-saving Percentage,
width=7cm, height=4cm,
legend style={at={(0.5,-0.5),font=\footnotesize},
anchor=north,legend columns=-1},
%symbolic x coords={14,15,16,17},
xtick=data,
%x tick label style={rotate=35,anchor=east},
%ytick={-20,-10,0,10,20},
minor ytick={0},grid=minor,
yticklabel={\pgfmathprintnumber\tick\%}
]
\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[y error=error]
{
x y error
14	23.45	0.66
15	11.29	0.30
16	-5.82	-0.06
17	-3.30	-0.04
};

\addplot+[
error bars/.cd,
x dir=both, x explicit,
y dir=both, y explicit,
]
table[y error=error]
{
x y error
14	22.85	0.00
15	10.25	0.00
16	-4.99	0.00
17	-2.08	0.00

};

\legend{Measurement,Model Estimation} 
\end{axis}
\end{tikzpicture}
\caption{BFS Energy-saving by Race-to-halt. This diagram shows how many percentages of energy-saving if executing BFS with 8 cores instead of 1 core. The positive percentages at scale 14 and 15 mean that RTH should be applied. The negative percentages at scale 16 and 17 mean that RTH should not be applied. The standard deviation of BFS energy-saving percentage is less than 3\%, from scale 14 to 17.}
\label{fig:BFS-RTH}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%
\comm{
\section{Related Work}
\label{sec:RelatedWorks}
The most similar work of our study is the Roofline model of energy \cite{Choi2013,Choi2014}. Although the Roofline model also considers algorithmic and platform properties, Roofline model conducts the experiments and identifies the parameters by running each system with its maximum number of cores. Therefore, it can not estimate the power consumption of a program running with a single or a certain number of cores. %The models proposed in this study considers the number of core as a parameter and be able to estimate power consumption for an application running with a certain number of cores.
Study by Alonso et al. \cite{Alonso2014} has provided an accurate energy model for the three specific dense matrix factorizations. %The model is specific for dense consider energy consumption of application tasks of three key dense-matrix as the model parameters. 
The model is built to estimate energy consumption for each task of the three key dense-matrix factorizations by identifying the model parameters for each application task.
%This makes the model less general to apply to other applications. The study devises the model for each type of tasks which are not general for any application. 
%RTHpower models, on the other hand, characterize applications by their operational intensities. Moreover, RTHpower models are devised based on measurement data from a set of micro-benchmarks. The experimental results are the training data to identify the average active cores $m$, power contention $P^{ctn}$ and time ratio $\alpha$ of the platform for each application operational intensity. %Both the model by Alonso et al. and RTHpower models do not require the access to power counters of the target platform. 
Korthikanti et al. \cite{Korthikanti2009, Korthikanti2010} proposes an theoretical energy model to find the optimum number of cores for a given application. %From our understanding, their energy model assumes that computation work and data access occur in sequential order which is not the case in real systems. The current systems can perform both computation and accessing data in parallel manner. 
The model, however, only provides theoretical background and make assumptions to find optimal number of cores without evaluating the model on real platforms yet.

Recently, real-time approaches have been developed to find the best configurations to run applications in order to achieve energy efficiency. Imes et al \cite{7108419} propose a portable approach to choose the running configuration to minimize energy consumption under real-time constraints. However, the approach must be applied on a platform that support changing configuration during run-time. It also requires platforms to have hardware resource providing power data that software can access. The ULP system studied in this work is not supported with the mentioned features. Mishra et al \cite{Mishra:2015} combines online and offline techniques to find the most energy-efficient configuration. However, this approach requires a significant amount of data collected to feed to its probabilistic network. This leads to a big overhead for short-time applications. Koala model \cite{Snowdon:2009} requires the system supported DVFS and short frequency switching delay in order to gain energy saving from its methodology. 
%Even though Koala model is validated with 10 platforms, 
Only two x86-based platforms among 10 validated platforms gain energy saving results which are presented in the paper. %Study by Woo et al. \cite{Woo:2008:EAL:1495784.1495841} focuses on finding how many cores should be built inside a chip to achieve the best energy efficiency. This helps chip designers to make decisions. Our models helps to identifying how many cores to run an application on a given embedded system to consume the least energy.
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Conclusion}
In this study, new fine-grained power models have been proposed to support architecture-application co-design. The models provide insights into how a given application consumes power when executing on an ultra-low power embedded system by considering both platform and application properties. The models have been validated on Movidius Myriad1, an ultra-low power embedded platform with data from 35 micro-benchmarks and three application kernels. We have also shown that by using the models, we can predict whether the race-to-halt strategy (RTH) is energy-efficient for a given application on a ULP embedded system. We have presented real scenarios when to use RTH and the framework based on the models could predict the scenarios precisely.
%Based on the models, we have devised a new framework to predict whether RTH is applicable to a given application on ULP embedded systems. The framework has been validated by both micro-benchmarks and application kernels. 
Improving and applying the models and framework to other embedded platforms (e.g., ARM) and other application kernels are parts of our future work.     
\comm{
The extendable works that we want to address in the future, are listed below.
\begin{itemize}
\item Apply the models to other platforms using the similar procedure. We want to validate and improve the models on other embedded platforms.
\item Apply the models to other application kernels in Berkeley dwarfs which represent the most common communication patterns. By considering the communication patterns of Berkeley dwarfs, we want to provide the more accurate power estimation for a wide range of real-world applications.
\item Build a run-time system using RTHpower models as a cost metric and RTH prediction framework to find the number of cores for running an application in order to improve energy efficiency. The run-time system will make decision based on platform properties, application properties and its input size.
\end{itemize}
}

==> uit-power-motiv.tex <==
The energy efficiency of computing systems can be enhanced via power models that provide insights into how the systems consume power. However, there are no application-general, fine-grained and validated power models which can provide insights into how a given application running on an ultra-low power (ULP) embedded system consumes power. %and, particularly, whether the race-to-halt strategy, an widely-used energy-efficient approach in high-performance computing systems, is still applicable to ultra-low power embedded systems. 

In this study, we devise new fine-grained power models that provide insights into how a given application consumes power on an ULP embedded system. The models support architecture-application co-design by considering both platform and application properties. The models are validated with data from 35 micro-benchmarks and three application kernels, namely dense matrix multiplication, sparse matrix vector multiplication and breadth first search, on Movidius Myriad, an ultra-low power embedded system. The absolute percentage errors of the model are at most 8.5\% for micro-benchmarks and 12\% for application kernels. Based on the models, we propose a framework predicting when to apply race-to-halt (RTH) strategy (i.e., running an application with a maximum setting) to a given application. For the three validated application kernels, the proposed framework is able to predict when to use RTH and when not to use RTH precisely. The experimental results show that the prediction of our new RTH framework is accurate and we can save up to 61\% energy for dense matrix multiplication, 59\% energy for sparse matrix vector multiplication by using RTH and 5\% energy for breadth first search by \emph{not} using RTH.
